Multi-Modal Gaze Following in Conversational Scenarios

Gaze following estimates gaze targets of in-scene person by understanding human behavior and scene information. Existing methods usually analyze scene images for gaze following. However, compared with visual images, audio also provides crucial cues for determining human behavior.This suggests that we can further improve gaze following considering audio cues. In this paper, we explore gaze following tasks in conversational scenarios. We propose a novel multi-modal gaze following framework based on our observation ``audiences tend to focus on the speaker''. We first leverage the correlation between audio and lips, and classify speakers and listeners in a scene. We then use the identity information to enhance scene images and propose a gaze candidate estimation network. The network estimates gaze candidates from enhanced scene images and we use MLP to match subjects with candidates as classification tasks. Existing gaze following datasets focus on visual images while ignore audios.To evaluate our method, we collect a conversational dataset, VideoGazeSpeech (VGS), which is the first gaze following dataset including images and audio. Our method significantly outperforms existing methods in VGS datasets. The visualization result also prove the advantage of audio cues in gaze following tasks. Our work will inspire more researches in multi-modal gaze following estimation.

==> tbl/quantitative/item.tex <==
% Please add the following required packages to your document preamble:
% \newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table}
\begin{center}
\caption{VideoGazeSpeech Dataset Summary Statistics}
\label{table2}
\resizebox{\linewidth}{!}{
\begin{tabularx}{\linewidth}{l | C}
\toprule
\textbf{Parameter} & \textbf{Value}  \\ 
\midrule
Total frame number      & 35231 \\
Duration for each video & ≈20 s          \\ 
Fps for each  video     & 25             \\ 
Size for each  video    & 1280*720      \\ 
Dataset Size            & 7.2GB           \\ 
\midrule

\end{tabularx}
}
\end{center}
\end{table}

==> tbl/quantitative/table3.1.tex <==
% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table}[t]
\begin{center}
\caption{Performance of Gaze Candidate Estimation Network with different backbones  in the AP metric$\uparrow$ (higher is better)}
\label{table3}
  \small
  % \footnotesize
  % \normalsize
\resizebox{\linewidth}{!}{%
\begin{tabularx}{\linewidth}{l | C C C }
\toprule
% Feature Map 
\multirow{2}{*}{\textbf{Feature Map }}
& $\mathbf{R_{101}}$ & $\mathbf{R_{50}}$ & $\mathbf{X_{101}}$ \\
   &\textbf{(AP)} &\textbf{(AP)}&\textbf{(AP)} \\
\midrule
Visual Feature & 0.420                  & 0.422               & 0.426                             \\
% Only Head   Position             & 0.432                  & 0.422               & 0.433                            \\
\textbf{Audio-Vision Feature~$\uparrow$}     & 0.425                & 0.430               & \textbf{0.433~$\uparrow$ }                       \\
\midrule

\end{tabularx}%
}
\end{center}
\end{table}

==> tbl/quantitative/table3.tex <==
% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}


 
  % \footnotesize
  % \normalsize
   


\begin{table}[t]
	\setlength\tabcolsep{8pt}
	\renewcommand\arraystretch{1.2}
	\centering
	\normalsize
	\caption{Performance of Gaze Candidate Estimation Network with different backbones  in the AP metric$\uparrow$ (higher is better)}
    \label{table3}

	\begin{tabular}{l|c|c}
        \toprule
        % Feature Map 
        \diagbox{Backbone}{Modality} & Vision & Vision and Audio\\
        \hline
        $\mathbf{ResNet-101}$ & 0.420 & 0.425~$\uparrow$  \\
        $\mathbf{ResNet-50}$& 0.422  & 0.430~$\uparrow$  \\
        $\mathbf{ResNeXt-101}$ & 0.426   & 0.433~$\uparrow$ \\
                                            
        \bottomrule
	\end{tabular}
	
\end{table}

% \begin{table}[t]
% 	\setlength\tabcolsep{8pt}
% 	\renewcommand\arraystretch{1.2}
% 	\centering
% 	\normalsize
% 	\caption{Performance of Gaze Candidate Estimation Network with different backbones  in the AP metric$\uparrow$ (higher is better)}
%     \label{table3}
% \small
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.48\textwidth}{!}{
%      \begin{tabular}{l|c|c|c|c|c|c}
%      \toprule
%      \multirow{2}{*}{\textbf{\diagbox{Backbone}{Modality}}} &\multicolumn{3}{c|}{\textbf{Vision}}&\multicolumn{3}{c}{\textbf{Vision + Audio}}  \\
%       &AUC & L^2 & mAP &AUC & L^2 & mAP  \\
%      \midrule
%    {ResNet-101}&&&0.420&&&0.425~$\uparrow$ \\
%    {ResNet-50}&&&0.422&&&0.430~$\uparrow$\\
%    {ResNeXt-50}&&&0.426&&&0.433~$\uparrow$\\

%      \bottomrule
%     \end{tabular}
% }
% \end{table}

==> tbl/quantitative/table4.1.tex <==
% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table}[t]
\begin{center}
\caption{Quantitative evaluation in comparison with state-of-the-art methods on our VGS dataset in the AP metric $\uparrow$ (higher is better). Our method outperforms DETR~\cite{zhu2020deformable} and VideoAttentionTarget~\cite{chong2020detecting}.

}
\label{table4}
 % \small
  % \footnotesize
  \normalsize
\resizebox{\linewidth}{!}{%
\begin{tabularx}{\linewidth}{l | C C C}
\toprule
\textbf{Feature   Map}   & 
% \textbf{Ours} & 
\textbf{\cite{zhu2020deformable}} & \textbf{\cite{chong2020detecting}} &
\textbf{Ours}\\
   % &(AP)&(AP)&(AP) \\ 
\midrule
Visual Feature                   & 0.400               & 0.3278      & 0.426                       \\
% Only Head   Position                             & 0.391               & 0.3297          & 0.433                     \\
\textbf{Audio-Vision Feature}                    & \textbf{0.418}               & \textbf{0.3244}    & \textbf{0.433}                          \\
\midrule

\end{tabularx}
}
\end{center}
\end{table}

==> tbl/quantitative/table4.tex <==
% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}


 
  % \footnotesize
  % \normalsize
   


\begin{table}[t]
	\setlength\tabcolsep{8pt}
	\renewcommand\arraystretch{1.2}
	\centering
	\normalsize
	\caption{Quantitative evaluation in comparison with state-of-the-art methods on our VGS dataset in the AP metric $\uparrow$ (higher is better). Our method outperforms DETR and VAT.}
    \label{table4}

	\begin{tabular}{l|c|c}
        \toprule
        % Feature Map 
        \diagbox{Network}{Modality} & Vision & Vision and Audio\\
        \hline
        VAT\cite{chong2020detecting} & 0.328 & 0.324~$\uparrow$  \\
        DETR\cite{zhu2020deformable}& 0.400  & 0.418~$\uparrow$  \\
        \textbf{Ours} & 0.426   & 0.433~$\uparrow$ \\
                                            
        \bottomrule
	\end{tabular}
% \small
% \setlength{\tabcolsep}{4pt}
% \resizebox{0.48\textwidth}{!}{
%      \begin{tabular}{l|c|c|c|c|c|c}
%      \toprule
%      \multirow{2}{*}{\textbf{\diagbox{Network}{Modality}}} &\multicolumn{3}{c|}{\textbf{Vision}}&\multicolumn{3}{c}{\textbf{Vision + Audio}}  \\
%       &AUC & L^2 & mAP &AUC & L^2 & mAP  \\
%      \midrule
%    VAT\cite{chong2020detecting}&0.718&0.230&0.328&0.736&0.235 &0.324~$\uparrow$\\
%     DETR\cite{zhu2020deformable}&&&0.400&0.751&206.58&0.418~$\uparrow$\\
%     \midrule
%     Ours& & &0.426&0.742&193.58&0.433~$\uparrow$\\

%      \bottomrule
%     \end{tabular}
% }
\end{table}



